Verifying OpenJDK's LinkedList using KeY

As a particular case study of the formal verification of state-of-the-art, real software, we discuss the specification and verification of a corrected version of the implementation of a linked list as provided by the Java Collection framework. Keywords: Java, standard library, deductive verification, KeY, Java Modeling Language, case study, bug

==> old/old_2_spectech.tex <==
\subsection{\label{subsec:spectech}Specification techniques}
We shall now discuss the main specification techniques that we employ in KeY: instance invariants, heap invariance, pure methods, and ghost fields. This discussion is incomplete, as there are other specification techniques which we do not treat here.

Every class or interface in Java can be annotated using JML's instance invariants. An instance invariant is a predicate that holds for a particular instance of the Java type that is annotated. After the constructor of a class completes, it is required to establish that the instance invariant holds. Moreover, for most method contracts, one requires that the instance invariant of the implicit \texttt{\textbf{this}} reference holds before the specified method is invoked, and it (re)established that the invariant holds after the method completes. Invariants are inherited; the instance invariant of a super interface or super class also holds for all instances of its subtypes.

Instance invariants are not always automatically enforced, and thus requires attention when specifying method contracts. For example, it is possible to modify the public fields of an instance in such a way that its instance invariant is broken. Moreover, for the default and unannotated constructor, KeY does not generate a proof obligation that the invariant must hold after object creation. For method parameters of reference type, the invariant is not assumed to hold. In this case, the JML operator {\jml \bs invariant\_for} can be explicitly stated in the pre- and post-condition. For methods that are declared as {\jml helper} it is not assumed that the instance invariant for \texttt{\textbf{this}} holds, nor is it required to show that its invariant holds after the method completes.

For example, consider the following (part of a) program:\\[5pt]
\texttt{\textbf{public final class} Example5 \{}\\
\-\hspace{10pt}\texttt{\textbf{public}} {\jml nullable} \texttt{Example5 next;}\\
{\jml\-\hspace{10pt}public instance invariant \texttt{next} == \texttt{\textbf{null}} || \texttt{next} != \texttt{\textbf{this}};}\\
\-\hspace{10pt}$\ldots$\\[5pt]
This specifies the instance invariant that the \texttt{next} field may either be \texttt{\textbf{null}}, or if it is non-null that it is not equal to the \texttt{\textbf{this}} reference. For this to work it is important to annotate the field as {\jml nullable}, since by default every field or parameter is assumed to be non-null. Next, we annotate the constructor:\\[5pt]
{\jml\-\hspace{10pt}behavior\\
\-\hspace{10pt}requires true;\\
\-\hspace{10pt}signals\_only \bs nothing;}\\
\-\hspace{10pt}\texttt{\textbf{public} Example5() \{\}}\\[5pt]
The method contract for the constructor does not explicitly mention that the invariant must be established after the constructor completes; this is added automatically. Since each field of reference type is, by the Java semantics, assigned to \texttt{\textbf{null}} even before the constructor is executed, establishing our instance invariant is easy.

An important aspects of specifying method contracts is heap invariance. This is captured by the \emph{assignable} clause of a JML contract. Over the course of executing the method, locations on the heap may be accessed and modified. Consider the situation in Figure \ref{fig:method_heap} again: in heap $H_2$, before executing the method, we may have established a property that holds for certain values on part of the heap. However, when the method is called and the heap after method completion is considered, the heap may have been modified that invalidates our earlier property. The {\jml assignable} clause allows us to show that certain properties are preserved by method calls: properties that holds for values on parts of the heap that are never touched by a method remain invariant under that method. In other words, a property that only depends on heap locations that are not assigned by the method, remain valid after the method completes. Consider these methods in \texttt{Example5}:\\[5pt]
{\jml\-\hspace{10pt}behavior\\
\-\hspace{10pt}requires \bs invariant\_for(\texttt{x}) \&\& \texttt{\textbf{this}} != \texttt{x};\\
\-\hspace{10pt}ensures \bs invariant\_for(\texttt{x}) \&\& \texttt{next} == \texttt{x};\\
\-\hspace{10pt}signals\_only \bs nothing;\\
\-\hspace{10pt}assignable next;}\\
\-\hspace{10pt}\texttt{\textbf{public void} linkNext(Example5 x) \{next = x;\}}\\
{\jml\-\hspace{10pt}behavior\\
\-\hspace{10pt}requires \bs invariant\_for(\texttt{a}) \&\& \bs invariant\_for(\texttt{b}) \&\& \texttt{a} != \texttt{b};\\
\-\hspace{10pt}ensures \bs invariant\_for(\texttt{a}) \&\& \bs invariant\_for(\texttt{b});\\
\-\hspace{10pt}signals\_only \bs nothing;}\\
\-\hspace{10pt}\texttt{\textbf{public static void} t(Example5 a, Example5 b) \{}\\
\-\hspace{20pt}\texttt{a.linkNext(b); b.linkNext(a);}\\
\-\hspace{20pt}\texttt{\textbf{assert} a.next == b \&\& b.next == a; \}\}}\\[5pt]
Here, we can prove the assertion of method \texttt{t} because we know: the invariant for \texttt{a} and \texttt{b} holds initially, and is preserved by \texttt{a.linkNext(b)} and \texttt{b.linkNext(a)}. Moreover, after we have assigned \texttt{a}'s \texttt{next} field in the first method invocation, this field is left unmodified by the second method invocation to \texttt{b.linkNext(a)}. Finally, we remark that the JML contract for \texttt{linkNext} is not marked by {\jml helper}, hence we implicitly have the requirement that {\jml\bs invariant\_for(\texttt{\textbf{this}})} holds before the method call and is ensured after it completes.

(strictly) pure methods

ghost fields

==> old/old_3_bottomup.tex <==
\subsection{\label{subsec:bottomup}Bottom-up specification}
Design specification to support specific class implementation

LinkedList instance invariant

Chain of nodes

Example: addFirst() method

Ghost parameters

Example: remove() method

==> old/old_4_topdown.tex <==
\subsection{\label{subsec:topdown}Top-down specification}
Design specification to support wide-range of interface implementations

model fields

Iterator

Collection (multiset)


==> section/3/1_key.tex <==
%\subsection{\label{subsec:key}An introduction to KeY}
%The \emph{KeY system} consists of three main components: a multi-sorted classical first-order sequent calculus with a large rule set, a translator of annotated Java programs into proof obligations, and an interactive tool for manipulating proofs.
\paragraph{Dynamic logic}
The logic underlying KeY is \emph{JavaDL}, a program logic that directly incorporates Java language features.
The program logic is a multi-modal logic: $\langle P\rangle\varphi$ means that executing the program fragment $P$ terminates and $\varphi$ holds in the final state; and $[P]\varphi$ means that \emph{if} the program fragment $P$ terminates, \emph{then} $\varphi$ holds in the final state. The formula $\varphi\to\langle P\rangle\psi$ means that if $\varphi$ holds in the initial state, then execution of $P$ terminates in a state for which $\psi$ holds. 
%See Chapter 3 of~\cite{ahrendt2016deductive} for more detail of JavaDL's syntax and semantics. we proceed with  summary of the matter important to us.

The program logic distinguishes \emph{program variables} from \emph{logical variables}: the value of a program variable can be changed over the course of executing a program, whereas a logical variable always has the same value.
%As a notation convention, program variables and fragments are written by a typewriter, and logical variables are italic.
% For example, $\mathtt{i},\mathtt{j}$ are program variables (of integer sort) and $z$ is a logical variable (also of integer sort). Then the formula $$\mathtt{i}=z\to\langle\mathtt{j=i;i=1;i=j\pp;}\rangle\mathtt{i}=z$$ means that execution of the program fragment terminates and the value of $\mathtt{i}$ is the same in the initial and the terminal state.
As logical variables can never be modified by a program fragment, they are used as so-called \emph{freeze variables}.

The proof system that KeY uses to establish validity of formulas is given as a sequent calculus. A sequent $\varphi_1,\ldots,\varphi_n \Rightarrow \psi_1,\ldots,\psi_m$ consists of $n$ antecendents and $m$ succedents, all formulas of JavaDL. Next to the rules for classical first-order logic, the proof system also consists of a large number of other rules. The large rule set is given by means of lightweight tactics (called taclets \cite{beckert2004taclets}) that perform modifications on the sequent one is proving: e.g.~spawn new branches, substitute variables, rewrite terms, or close a branch. There are approximately 1750 rules that implement Java program semantics and allow for symbolic execution, and implement the theories of many sorts: integers, sequences, heaps, location sets, and others.

Of particular interest to us are rules concerning \emph{updates} and \emph{heaps}. There are rules that transform modalities with program fragments into so-called update modalities. Updates always terminate and they assign JavaDL terms to program variables. As such, updates cannot assign program variables to side-effectful expressions. Given a formula $\varphi$, then $\{\mathtt{x}_1\coloneqq t_1||\ldots||\mathtt{x}_n\coloneqq t_n\}\varphi$ is a formula where in parallel $\mathtt{x}_i$ are updated to $t_i$.

%Moreover, as program variables have an integer sort that is interpreted as the standard infinite set of integers, Java integer expressions must be translated to correctly model integer overflow (Section 5.4.3 of \cite{ahrendt2016deductive}).

%To prove the validity of a formula, we create a sequent with only that formula as succedent. If rule applications lead to branches which are all closed, the formula is proven. Part of the proof of our previous example is shown in Figure~\ref{fig:example_proof}.
%
%\begin{figure}
%$$\infer[\mathsf{impRight}]{
%\Rightarrow \mathtt{i}=z\to\langle\mathtt{j=i;i=1;i=j\pp;}\rangle\mathtt{i}=z
%}{\infer[\mathsf{assign}]{
%\mathtt{i}=z \Rightarrow \langle\mathtt{j=i;i=1;i=j\pp;}\rangle\mathtt{i}=z
%}{\infer[\mathsf{assign}]{
%\mathtt{i}=z \Rightarrow \{\mathtt{j}\coloneqq\mathtt{i}\}\langle\mathtt{i=1;i=j\pp;}\rangle\mathtt{i}=z
%}{\deduce[\vdots]{
%\mathtt{i}=z \Rightarrow \{\mathtt{j}\coloneqq\mathtt{i}\}\{\mathtt{i}\coloneqq\mathtt{1}\}\langle\mathtt{i=j\pp;}\rangle\mathtt{i}=z
%}{\vspace{-4pt}\infer[\mathsf{simp}]{
%\mathtt{i}=z \Rightarrow \{\mathtt{j}\coloneqq\mathtt{i}\}\{\mathtt{i}\coloneqq 1\}\{\mathtt{i}\coloneqq\mathtt{j}||\mathtt{j}\coloneqq\mathtt{j}\oplus1\}\langle\rangle\mathtt{i}=z
%}{\infer[\mathsf{empty}]{
%\mathtt{i}=z \Rightarrow \{\mathtt{j}\coloneqq\mathtt{i}\}\{\mathtt{i}\coloneqq 1\}\{\mathtt{i}\coloneqq\mathtt{j}\}\langle\rangle\mathtt{i}=z
%}{\infer[\mathsf{applyUpd}]{
%\mathtt{i}=z \Rightarrow \{\mathtt{j}\coloneqq\mathtt{i}\}\{\mathtt{i}\coloneqq 1\}\{\mathtt{i}\coloneqq\mathtt{j}\}\mathtt{i}=z
%}{\infer[\mathsf{simp}]{
%\mathtt{i}=z \Rightarrow \{\mathtt{j}\coloneqq\mathtt{i}\}\{\mathtt{i}\coloneqq 1\}\mathtt{j}=z
%}{\infer[\mathsf{applyUpd}]{
%\mathtt{i}=z \Rightarrow \{\mathtt{j}\coloneqq\mathtt{i}\}\mathtt{j}=z
%}{\infer{
%\vphantom{\{}\mathtt{i}=z \Rightarrow \mathtt{i}=z
%}{\vspace{0pt}}}}}}}}}}}$$
        %\caption{Example of part of a proof in JavaDL.}
        %\label{fig:example_proof}
%\end{figure}
%
%Here, the $\mathsf{impRight}$ rule comes from standard classical sequent calculus. The assignment rule transforms the program modality into an update modality. The empty rule removes the empty program modality. The function $\oplus$ models Java's overflow behavior on \texttt{int}. The simplification rule removes any update that has no effect on the formula on its right. Only the right-most updates can be applied to the formula.

==> section/3/2_heaps.tex <==
%\subsection{\label{subsec:key-heaps}Heaps and Objects}
\paragraph{Data types}
There is a hidden and implicit program variable in JavaDL that is the \texttt{heap} of heap sort. The heap is used to model the storage of objects, that is, the value of fields associated to object references. From a practical perspective, updates of program variables other than the heap can be thought of as stack variables. Such program variables can \emph{refer} to objects on the heap. Heap updates are reflected by updating the \texttt{heap} program variable. Heap updates and program variable updates easily form complex expressions, where both kinds of updates can be intertwined: we do not show heap update expressions here, but see Section 2.4.3 and Section 6.4 of \cite{ahrendt2016deductive}.

Next to the built-in sorts of integers, sequences, heaps, and location sets, are Java types. Each Java type has its own sort in JavaDL that models (infinitely many) references to objects, including the \texttt{\textbf{null}} reference. References can be explicitly coerced between sorts, to model subtypes: e.g. every reference can be coerced to a reference of sort \texttt{Object}. A heap assigns values to the fields of a non-null reference.
Object references are global, but the creation status of each object is a special Boolean field \texttt{<created>} local to each heap. An object becomes created in some heap by taking a fresh reference, that has no value yet assigned to its creation field in that heap, and setting that field to \texttt{\textbf{true}}. Fields can only be assigned to non-null object references for which their created field is true.
%A similar field, \texttt{<initialized>}, exists that reflects whether the constructor call is completed.
A heap is \emph{well-formed} if a finite number of references have \texttt{<created>} set to true.
%For example, consider a class \texttt{Example2} with precisely one field: \texttt{ref} of reference type to \texttt{Object}:\\[5pt]
%\texttt{\textbf{public class} Example2 \{ \textbf{public} Object ref; \}}\\[5pt]
%and let \texttt{a} be a program variable of sort \texttt{Example2}:
%\begin{gather*}
%\langle\mathtt{a}=\boldsymbol{\mathtt{new}}\mathtt{\ Example2();\ a.ref=a;}\rangle\\[-4pt]
%\mathtt{a.ref}=\mathtt{((Example2)\ a.ref).ref}
%\end{gather*}
%This program fragment creates a new object, and assigns its \texttt{ref} field to itself. After the fragment terminates, the \texttt{Object} reference of \texttt{ref} is casted to \texttt{Example2} and it's \texttt{ref} equals that of the object referred by program variable \texttt{a}. One can check that this formula is provable in KeY.\footnote{See Appendix \ref{sec:proofs}, Example 2: our proof in KeY has 167 steps and 3 branches.}

%When creating multiple objects it is important to discriminate their identities. As one object is created before the other, there is a time in which the older object has \texttt{<created>} set, while the new object has no \texttt{<created>} set yet, allowing us to make a distinction between the two references. However, this is only possible if the heap has a finite number of created objects. So to enable us to deduce that a fresh reference is not equal to any existing reference, it is required that heap is \emph{well-formed}: only a finite number of references have \texttt{<created>} set to true.
%Consider this example:\\[5pt]
%\texttt{\textbf{public class} Example3 \{\}}\\[5pt]
%and let \texttt{a} and \texttt{b} be both program variables of sort \texttt{Example3}:
%\begin{align*}
%\langle\mathtt{a}=\boldsymbol{\mathtt{new}}\mathtt{\ Example3();\ b}=\boldsymbol{\mathtt{new}}\mathtt{\ Example3();}\rangle\mathtt{a}\neq\mathtt{b}
%\end{align*}
%Without the premise $\mathsf{wellFormed}(\mathtt{heap})$, it is not possible to prove that \texttt{a} and \texttt{b} are different references after the program fragment. However, neither is it possible to prove that \texttt{a} and \texttt{b} are the same. Above formula is a contingency.

%\begin{figure}
 %   \centering
 %   \includegraphics{section/3/method_heap.eps}
 %   \caption{Heaps are `threaded' through method calls. In heap $H_1$ the program fragment $P$ is executed, resulting in heap $H_2$. Either a contract for method \texttt{m()} is employed, which relates the before heap $H_b$ to some heap after the method call $H_a$; or, the method body is unfolded wrapped in a method frame that resolves overshadowing of program variables. In both cases, to call the method, heap $H_b$ is equal to $H_2$ and heap $H_a$ is equal to $H_4$. Then the program fragment $P'$ that occurs after the method call is executed using the heap returned by the method.}
    \label{fig:method_heap}
%\end{figure}


==> section/3/3_jml.tex <==
%\subsection{\label{subsec:key-methods}Methods and JML}
%\paragraph{Methods and JML}
\paragraph{JML}
%An important aspect of Java programs are method calls. There are three main issues: calling a method may introduce new program variables that overshadow older program variables, calling a method may change the heap, and it is possible to call a method on an object for which its exact type is only known at run-time.
%To solve the issue of overshadowing older program variables, KeY uses \emph{method frames}; before a method frame is created, it is ensured that old program variables and new program variables do not collide by renaming the program variables of a method body. Since the \texttt{\textbf{this}} keyword cannot be renamed, the method frame provides a context in which program fragments evaluates \texttt{\textbf{this}} references; it also tracks where the method return value must be placed. The heap supplied to the method call is the heap as it was after the statements that occurred before the method call, and statements following a method call are performed using the heap as it is after the method call completes: there are rules for `threading' the heap through a method call, see Figure \ref{fig:method_heap}. There are roughly two ways of treating method calls: unfolding their method body wrapped in a method frame, or using its method contract.
Method contracts and general annotations of Java programs
are specified in terms of a subset of the Java Modeling Language (JML)~\cite{leavens2013jml} but with KeY-specific extensions, see \cite{huisman2014jml} or Chapter 7 of~\cite{ahrendt2016deductive}. This allows the use of KeY for post-hoc verification: after a program has been developed and validated, classes and their members are annotated. In particular, each method is annotated by a contract that specifies pre- and post-conditions. In this approach, methods are the central point of our verification effort. Its annotations determine their correctness formulas in JavaDL: if they are verified, then the corresponding method is correct with respect to its method contract. Consequently, method contracts can be reused in other proofs involving program fragments that call such method.

%As an example program annotation with JML, consider:\\[5pt]
%\texttt{\textbf{public class} Example4 \{}\\
%\-\hspace{10pt}\texttt{\textbf{public} Example4 ref;}\\
%\-\hspace{10pt}\texttt{\textbf{public final void} set(Example4 a) \{}%
%\texttt{ref = a.ref;}%
%\texttt{\}}\\
%{\jml\-\hspace{10pt}behavior\\
%\-\hspace{10pt}requires true;\\
%\-\hspace{10pt}signals\_only \bs nothing;}\\
%\-\hspace{10pt}\texttt{\textbf{public static void} test() \{}\\
%\-\hspace{20pt}\texttt{Example4 a = \textbf{new} Example4();}\\
%\-\hspace{20pt}\texttt{Example4 b = \textbf{new} Example4();}\\
%\-\hspace{20pt}\texttt{b.ref = a; a.set(b);}\\
%\-\hspace{20pt}\texttt{\textbf{assert} a.ref == a \&\& b.ref == a;}
%\texttt{\}\}}\\[5pt]
%The blue text forms a JML annotation: it states that the behavior of this method, under any precondition ({\jml requires true}), completes normally ({\jml signals\_only \bs nothing}). Loading this into KeY generates a corresponding proof obligation. The first steps are similar to our previous example where we allocate two objects (assuming a well-formed heap). What is important here is that the \texttt{set} method is marked \texttt{\textbf{final}}, meaning there is no possible overriding method --- solving the issue that the exact type of an object is not known at run-time. This allows us to apply a rule for expanding the method call into its method body. The method body is wrapped in a method frame assigning \texttt{\textbf{this}} to \texttt{a} and the formal parameter \texttt{a} is replaced by a fresh program variable \texttt{a\_1} assigned to the actual parameter \texttt{b}, preventing overshadowing. Within the frame, we take the heap after allocation of the two objects, and we execute \texttt{\textbf{this}.ref = a\_1.ref}. The resulting heap is then passed back after the method frame is closed. Within the resulting heap, we consider the \texttt{\textbf{assert}} statement. There are proof rules that verify that its condition hold.\footnote{See Appenix \ref{sec:proofs}, Example 4: our proof has 674 steps and 14 branches.}

Other than method contracts, JML also allows annotations of ghost fields, model fields and model methods. Ghost fields are virtual fields that become part of the modelled state of an object on the heap, but are never present when actually executing a Java program. The value of ghost fields are assigned a default value at object initialization, and can be explicitly changed by JML \texttt{set} annotations. These annotations occur anywhere in method bodies where otherwise a normal statement can be expected. Model fields are introduced as function symbols, and several axioms are added that allow the definition of model fields to be employed during proof. An example model field is a \emph{class invariant}, which is implicitly assumed to hold of the state of an object between method invocations. More general than model fields are model methods: every model field is implemented as a specific model method. Other annotations, such as loop invariants, are also added to the method body: these are automatically applied by KeY's symbolic execution.

Java programs annotated with JML are entered into the KeY system and the verification of their correctness formulas begins, by generating one or more \emph{proof obligations} for each correctness formula. Using the interactive tool, a proof tree is constructed by applying rules until the branches of the tree are closed. Each rule application may result in zero or more branches: in the case of multiple branches, every branch needs to be closed. The tool also provides automation, that automatically applies proof rules using heuristics. This speeds up the verification effort considerably. Finally, after all proof obligations appear as the conclusion of a closed proof tree, the verification effort is done. The proof trees can be stored in a file and reloaded and inspected later.


==> section/3_formal.tex <==
\section{The Key approach to formal verification}
To formally specify and verify correctness of Java programs, we make use of KeY --- see \emph{The KeY Book} \cite{ahrendt2016deductive}. The \emph{KeY project} has evolved over time in the \emph{KeY system} that includes: an interactive proof environment (GUI), a translator of annotated Java programs, and a many-sorted first-order dynamic logic sequent calculus with a large rule set.
%
%Note that a major assumption is that we have no \emph{multi-threading}, i.e. we assume a single thread only. Multi-threading is not (fully) supported by KeY. Also, for our purpose, this is not a problem: the Java documentation explicitly mentions that the \texttt{LinkedList} implementation is not intended to be operated on by multiple threads simultaneously without external synchronization.
%
% \item The third major assumption is that we leave out user-defined object \emph{equality} from our consideration. In principle, the KeY system supports specifying the equality method for object instances. However, we consider the problem too difficult to tackle: especially when considering cyclic data structures, such as a \texttt{List} instance containing itself, it is unclear what even the definition of equality should be. In our effort, we replace all occurrences of \texttt{Object\#equals(Object)} by primitive referential equality that compares references.
% \item The last two minor assumptions are that we have a fixed maximum array size for Java arrays such as \texttt{Object[]}, and a fixed maximum number of objects that can exists simultaneously. We shall informally argue how to compute these values in Section \ref{sec:improved}.
%
%In section \ref{subsec:key}, we first shortly cover the basics of the KeY approach to formal specification and verification of Java programs, by introducing the Java Modeling Language (JML) and highlighting interesting aspects of JavaDL, the dynamic logic used by KeY. We introduce the specification techniques in section \ref{subsec:spectech} that we shall employ in specification of the classes and interfaces directly related to the \texttt{LinkedList} implementation we wish to verify, and refer to relevant literature for more in-depth coverage of these techniques. We then apply these techniques in three styles: \emph{bottom-up specification} (sec. \ref{subsec:bottomup}), where we start with \texttt{LinkedList} and specify sufficient properties that are needed to verify the implementation; and \emph{top-down specification} (sec. \ref{subsec:topdown}), where we start with \texttt{Collection} and \texttt{Iterator} interfaces and specify the necessary properties of implementors of these interfaces.
%
In this section we will give a brief introduction to KeY that serves as a high-level overview of the techniques applied by KeY.

